Intelligent Pooling: Proactive Resource Provisioning in Large-scale Cloud Service

The proliferation of big data and analytic workloads has driven the need for cloud compute and cluster-based job processing. With Apache Spark, users can process terabytes of data at ease with hundreds of parallel executors. At Microsoft, we aim at providing a fast and succinct interface for users to run Spark applications, such as through creating simple notebook "sessions" by abstracting the underlying complexity of the cloud. Providing low latency access to Spark clusters and sessions is a challenging problem due to the large overheads of cluster creation and session startup. In this paper, we introduce Intelligent Pooling, a system for proactively provisioning compute resources to combat the aforementioned overheads. To reduce the COGS (cost-of-goods-sold), our system (1) predicts usage patterns using an innovative hybrid Machine Learning (ML) model with low latency and high accuracy; and (2) optimizes the pool size dynamically to meet customer demand while reducing extraneous COGS. The proposed system auto-tunes its hyper-parameters to balance between performance and operational cost with minimal to no engineering input. Evaluated using large-scale production data, Intelligent Pooling achieves up to 43% reduction in cluster idle time compared to static pooling when targeting 99% pool hit rate. Currently deployed in production, Intelligent Pooling is on track to save tens of million dollars in COGS per year as compared to traditional pre-provisioned pools.

==> architecture.tex <==
\section{Implementation}
Implementation details, design principals and end-to-end architecture (wt Kusto, data transaction pipeline, etc.).
\subsection{High-Level Architecture}


==> designprincipal.tex <==

\subsection{Design Principals}
We consider three major requirements when designing the system:

\mypar{Incorporate system-level constraints}
            We design a live pool that maintains a constant number of clusters. Three system-level constraints need to be incorporated into its design:
            (1) to avoid throttling issues, the live pool should not submit a large number of re-hydration requests in a short period of time;  
            (2) the pool size should not be updated too frequently because this can result in the possible cancellation of cluster creation requests (in the case of decreasing pool size), which might not be cost-effective or feasible considering potential network latencies;
            (3) there should be a minimum and maximum for the pool size to act as guardrails to ensure we do not over- or under-hydrate the pool.
            
% \mypar{Consider cost-performance trade-offs} In the optimization, we want to balance between the cost and performance, while satisfying the performance requirement (e.g., less than 20 second's average waiting time).
% is satisfied and the corresponding operational cost is minimized. 

%\al{Figure 1 is outdated (we don't use a Job Submission Worker anymore to run the ML script. May need to sync on making an updated diagram.)}
%\al{In Figure 1, is it possible to make the font a little bigger in certain areas (e.g. Work Item Service and Generic Job Service) for readability?}\yz{Sure. Updated.}
\mypar{Scalability and efficiency} The system needs to be simple and maintainable, fast and adaptive to the real-time system status, and able to scale up to a large number of regions and potentially multiple pools with different cluster configurations (e.g., number of nodes, VM SKUs, etc.). Ideally, the optimal pool size can be updated every 5 min with the latest observation.

\mypar{Service Level Agreement (SLA) compliance} While minimizing the total COGS of the pool, with tuning knobs exposed to control the trade-off between performance and cost, we set a minimum requirement of the performance measured by the \textit{hit rate} (i.e., the percentage of clusters that can be acquired without on-demand initialization) that ensures that we reach a certain level of SLA. A robust model to ensure a certain service level is required.

\subsection{Deployment}
\al{TODO: Revisit this paragraph once we have it set up in PPE, Prod, etc.}
\sysname was set up for all regions of the \trident service, impacting a large number of clusters. While in production we:
(1) constantly run the optimization job(s) in a while loop to update the configuration in real-time with high frequency (every few seconds) to adapt to the latest system status, this is only feasible as we have optimized the end-to-end latency of the algorithm to mere seconds (see Sectcion~\ref{sec:exp});
(2) set up a guardrail to check on the ML model's prediction accuracy before running the downstream optimization. Specifically, we separate the input time series into train and validation, and use the validation for evaluation;
(3) set up alerting system for pipeline failures such that we can be noticed and investigate into any potential issues;
(4) create an exhaustive logging system around every step of the algorithm to allow monitoring and potentially debugging of the recommendation; and
(5) apply hyperparameter tuning for ML modules constantly as there is no one-fits-all solution with the dynamic changing pattern of the workloads.

